WalkieLokie: Relative Positioning for Augmented Reality Using a Dummy Acoustic Speaker

We propose and implement a novel relative positioning system, WalkieLokie, to enable more kinds of Augmented Reality applications, e.g., virtual shopping guide, virtual business card sharing. WalkieLokie calculates the distance and direction between an inquiring user and the corresponding target. It only requires a dummy speaker binding to the target and broadcasting inaudible acoustic signals. Then the user walking around can obtain the position using a smart device. The key insight is that when a user walks, the distance between the smart device and the speaker changes; and the pattern of displacement (variance of distance) corresponds to the relative position. We use a second-order phase locked loop to track the displacement and further estimate the position. To enhance the accuracy and robustness of our strategy, we propose a synchronization mechanism to synthesize all estimation results from different timeslots. We show that the mean error of ranging and direction estimation is 0.63m and 2.46 degrees respectively, which is accurate even in case of virtual business card sharing. Furthermore, in the shopping mall where the environment is quite severe, we still achieve high accuracy of positioning one dummy speaker, and the mean position error is 1.28m.

==> _ <==
\section{Synchronization and Ranging}

The distance estimation algorithm is not always accurate for all the walking lines, which is affected by the distance and signal strength, etc.
However, we find that the estimations can by synthesized if they are synchronized.
That is, in synchronization, the phone detects the receiving time of the periodical signal $s_2(t)$ and infers the different distances using the time\footnote{Note the difference between the displacement tracking by PLL and distance differencing by synchronization: the PLL is more accurate for real-time displacement tracking but has accumulated errors compared with synchronization.}. 
Hence, the more accurate distance can be obtained where we call this \textit{ranging} for differencing the previous \textit{estimation}.
The other benefit of synchronization is that once the calculated distance is accurate enough, the real-time distance can be obtained only using synchronization without the requirement of distance estimation again.

To design the synchronization signal $s_2(t)$ and the detection algorithm, several questions should be covered:
\begin{itemize}
    \item The acoustic bandwidth of one speaker should not be large in order to support more speakers in the room.
        First, the ideal configuration is that $s_1(t)$ and $s_2(t)$ of the speaker is at the same frequency band, which is being used in our proposal.
        Second, the bandwidth of $s_2(t)$ should be small. 
        However, it is challenging that the signal should take more bandwidth if $s_2(t)$ can be successfully detected.
    \item $s_2$ should also be capable of being used for displacement tracking. 
        
\end{itemize}






==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-huang}}]{Wenchao Huang}
received the B.S. and Ph.D degrees in computer science from University of Science and Technology of China in 2005 and 2011, respectively.
He is currently a Research Associate in School of Computer Science and Technology, University of Science and Technology of China. 
His current research interests include mobile computing, information security, trusted computing and formal methods.
\end{IEEEbiography}
\vspace{-0.6in}

%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-xiong}}]{Yan Xiong}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-xiong}}]{Yan Xiong}
received the B.S., M.S., and Ph.D degrees from University of Science and Technology of China in 1983, 1986 and 1990 respectively. 
    He is a professor in School of Computer Science and Technology, University of Science and Technology of China. 
    His main research interests include distributed processing, mobile computing, computer network and information security. 
\end{IEEEbiography}
%\vspace{-0.6in}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-xiangyang}}]{Xiang-Yang Li}
is a professor at the Illinois Institute of Technology.   Dr. Li received MS (2000) and PhD (2001) degree at Department of Computer Science from University of Illinois at Urbana-Champaign, a
Bachelor degree at Department of Computer Science and a Bachelor degree at Department of Business Management from Tsinghua University, P.R. China, both in 1995. His research interests include mobile computing, cyber physical systems, wireless networks, security and privacy, and algorithms. 
\end{IEEEbiography}
\vspace{-0.6in}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-yiqing}}]{Yiqing Hu}
 is a Ph.D. candidate in school of Computer
Science and Technology, University of Science and
Technology of China, His main research interests
include indoor localization, smart sensing and data
mining.
\end{IEEEbiography}
\vspace{-0.6in}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-xufei}}]{Xufei Mao}
received the Ph.D. degree in Computer Science from Illinois Institute of Technology, Chicago in 2010. He received the MS degree (2003) in Computer Science and the Bachelor degree (1999) in Computer Science at Northeastern University and Shenyang University of Technology respectively. 
He is with the School of Software and TNLIST, Tsinghua University, Beijing China. His research interests span wireless ad-hoc networks, wireless sensor networks, pervasive computing, mobile cloud computing and game theory.
\end{IEEEbiography}
\vspace{-0.6in}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-panlong}}]{Panlong Yang}
received his B.S. degree, M.S. degree, and Ph.D. degree in communication and information system from Nanjing Institute of Communication Engineering, China, in 1999, 2002, and 2005 respectively. Dr. Yang is now an associate professor in the PLA University of Science and Technology. Dr. Yang has published more than 50 papers in the areas of mobile ad hoc networks, wireless mesh networks and wireless sensor networks.
\end{IEEEbiography}

\vspace{-0.6in}

%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-xuangou}}]{Xuangou Wu}
    %Xuangou Wu received the Ph.D. degree in the school of Computer Science and Technology, University of Science and Technology of China, Hefei, China, in 2013. He is currently a lecture with the school of Computer Science and Technology, University of Anhui Technology, Ma'anshan, China. His research interests include wireless sensor networks, crowdsourcing and compressive sensing.
%\end{IEEEbiography}

\vspace{-0.6in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photoc-jumin}}]{Jumin Zhao}
    is a professor at college of information engineering of Taiyuan University of Technology (TUT), Shanxi, China. Dr. Zhao received Ph.D degree (2008) at Electronic Information College from TUT, a Bachelor degree at Electronic Information College and a Bachelor degree at Foreign Language college from TUT both in Jul. 1998. Her research interests include the signal processing, wireless networks, mobile computing, cyber-physical system, and algorithms.
\end{IEEEbiography}






==> tabstract_old.tex <==
\begin{abstract}
Ranging and direction estimation are not only the key methods in indoor localization, but also attractive to wider applications, such as social connectivities, fire rescuing, etc.
However, they require special hardwares as anchors and the implementation of both becomes more challenging.
In this paper, we propose \ourprotocol, the real-time ranging and direction estimation of the acoustic source using the smartphone.
\ourprotocol only requires that the source broadcasts the audio which is mixed with the non-audible signal. 
So the commercial off-the-shelf (COTS) speakers can serve as anchors.
The key insight under our paper is that when the user walks, the displacement pattern relatively from the user to the source is related to position of the source. 
We track the displacement using the second-order Phase Locked Loop that is accurate under weak signals.
We then estimate the position for each time the user walks in a line before turning.
We further propose the synchronization mechanism to synthesize all the estimations to enhance the accuracy and robustness when the user walks for longer steps.
Our extensive experiments show that the ranging and the direction estimation errors are under $0.66m$ and $5.06^o$ at the percentage of $90\%$ for most cases.

%Recent indoor localization techniques using the TOA or TDOA achieve high accuracy.
%However, they require specialized hardwares as anchor nodes which prevents the practical use of them.
%The main reason for the requirement is to implement synchronization among the anchors and smartphone to infer the traveling time of the signal, which corresponds to the distance from the phone to the anchor node.
%Hence, it is challenging to implement accurate synchronization with non-specialized hardwares.
%In this paper, we propose and implement the indoor localization by using the commercial off-the-shelf (COTS) speakers as anchor which are already installed in most public indoor places.
%The intuition under our design is that the distance can be estimated according to the difference of the relative displacement from the smartphone to the anchor node between each user's walking step.
%To solve the synchronization problem and get the accurate distance, the speaker broadcasts audios which are mixed with a modulated continuous signal.
%We leverage the signal to track the relative displacement and further estimate the course-grained real-time distance from the phone to the anchor when the user walks with the phone.
%Meanwhile, we use the signal for synchronization by synthesizing the former estimated distances and getting the accurate distance at each step.
%While the previous TOA or TDOA schemes requires multiple nodes for trilateration, our method also estimates the direction from the smartphone to the anchor such that we only require the minimum of one speaker for localization. 
%
\end{abstract}



==> tdiscussion.tex <==
\section{Discussion}
\subsection{Limitations}
In the preceding sections, we have presented and evaluated the \ourprotocol system.
\ourprotocol proposes a novel method to calculate the relative position, and currently 
there are some limitations as follows and we will address these challenges in our future work.

Since the relative displacement tracking of \ourprotocol is sensitive to NLoS effects, a user has to hold the phone in hand to get the relative position, and cannot put the phone in the pocket. 
Hence, it is more practical to install \ourprotocol on wearable devices, such as smartwatch 
\cite{samunggear,sonysmartwatch}
or smartglasses \cite{GoogleGlass}.
A possible improvement is to replace acoustic signals with WIFI signals, where there is much less attenuation of WIFI signals in case of NLoS effects.

\ourprotocol can immediately calculate precise distance from user to source when the distance from phone to source is within 8m, but needs historical precise measurements for ranging when the distance increases.
(Note that for direction estimation, there is no such limitation.)
For indoor localization, an easy solution is to place anchors at the place where users always pass through.
When users try to find nearby friend by \ourprotocol, since direction estimation is accurate without the requirement of synchronization, they can only use direction estimation when the friend is far away, and additionally use ranging when they are getting closer.

\subsection{Privacy Issue}
\ourprotocol shows new potential privacy attacks in mobile applications.
Recently, thousands of Android malwares have been identified in security community \cite{Zhou2012}. 
Most of the attacks are based on invalid use of permissions, such as SEND\_SMS (FakePlayer \cite{Fakeplayer}),
%(sending SMS to a premium-rate number without user awareness),
or ACCESS\_FINE\_LOCATION (Tapsnake \cite{tapsnake}).
Hence, many approaches aims at detecting and preventing undesirable usage of permissions \cite{Zhang2013,Yang2013}.
However, observe that the phone does not need any permissions to act as acoustic source or count walking steps using IMU sensors.
Furthermore, as our PLL tracks the relative displacement from acoustic source to receivers, \ourprotocol can also be used in a scene where the receivers, \eg, microphones, act as anchors.
Therefore, by emitting non-audible signals on the phone without user awareness and relative positioning by \ourprotocol, the phone's fine-grained location can also be obtained without the permission of ACCESS\_FINE\_LOCATION.



==> tintroduction_old.tex <==
\section{Introduction}

Many proposals on ranging \cite{2013-MobiSys-Guoguoenablingfine,Priyantha:2000:CLS:345910.345917,1097833,6566822, DBLP:conf/mobicom/HarterHSWW99} and directing estimation \cite{Joshi:2013:PLI:2482626.2482651,Xiong:2013:AFI:2482626.2482635, 4509717} have been proposed in indoor localization. 
They achieve considerable accuracy but require special hardwares as anchors or receivers.
The scheme that implements both techniques becomes a more challenging problem,
which also leads to a postponement of many attractive applications to be developed. 
For example, in mobile social networks, the user enters a cafe to make friends with nearby person whose online ID is bound to the position,
or the firefighters search and localize people where they are hard to yell for help due to the heavy smoke, etc.
%the mother tracks the position of the children in case of lost while shopping,
%or tourists keep updating the position of the guide that they feel free to enjoy the view or take photos, etc.
Until recently, some applications have tried the similar functions, such as Google's Latitude \cite{GoogleLatitude} and Facebook's Friendshake \cite{friendshake}, but they are mainly based on GPS and cannot track the people in indoor environments.

This paper introduces \ourprotocol, the first real-time ranging and direction estimation method that locates acoustic source using the smartphones.
The only requirement for the source is that the audio it broadcasts is mixed with non-audible signals.
Unlike the methods that range between phones\cite{2007-SenSys-BeepBeephighaccuracy,2011-SenSys-feasibilityrealtime}, the source does not need communication or computation capabilities.
Hence, commercial off-the-shelf (COTS) speakers can serve as anchors.
Compared to Swadloon \cite{DBLP:journals/corr/HuangXLLMYL13}, \ourprotocol achieves the real-time direction estimation that the user does not need to shake the phone when s/he wants to know the direction.
Moreover, \ourprotocol implements both ranging and direction estimation that using one anchor nodes.

The key insight of our paper is that when the user walks in a line, the pattern of the relative displacement from the user to the source is related to the position of the source.
For example in Figure \ref{fig:example}, the user walks and steps at $O_1$, $O_2$, and $O_3$.
The relative displacements $d_1=l_1-l_2$ and $d_2=l_2-l_3$ are measured and the user's walking length, \eg, $|\overline{O_1O_2}|$, is given.
Intuitively, $d_1\approx0$ which infers that $O_1$ and $O_2$ is close to $H$ where $\overline{AH} \bot \overline{O_1O_2}$ and $d_2<0$ which infers that the source is at the back of the walking user.
They infer the coarse-grained direction.
Another intuition is that when the distance $|\overline{AH}|$ becomes larger, $|d_2-d_1|$ becomes relatively smaller, which infers the coarse-grained distance.
Hence, the position of the source $A$ relative to the walking line $\overline{O_1O_3}$ can be estimated.
Moreover, if source serves as an anchor and its coordinate in the room is given, the real-time position of the user (\eg, $O_1$, $O_2$, $O_3$,\dots) can be inferred.
\begin{figure}[htpb]
    \vspace{-0.1in}
    \begin{center}
        \includegraphics{fexample-crop.pdf}
    \end{center}
    \caption{Example of relations between relative displacement and positions.}
    \label{fig:example}
    \vspace{-0.15in}
\end{figure}

As the displacement is small for each user's step and the step length of the user is not strictly constant, the practical challenge is to obtain the position when the user walks for very few steps in a line.
Especially when the user is far from the source, the measured displacement are more sensitive to noises and $|d_2-d_1|$ becomes much small that even tiny error in the measurement would cause large errors in positioning.
Hence, it requires accurate displacement measurement and robust locating algorithm.

To track the relative displacement, the source is mixed with a sine signal, and we use the phase locked loop (PLL) to track the phase of the signal, which corresponds to the displacement.
Unlike \cite{DBLP:journals/corr/HuangXLLMYL13} that uses the first order PLL for tracking the phase, we adopt the second order PLL which avoids jitters and shows improved accuracy when the signal is weak.
Then the distance and direction are estimated according to the relative displacement when the user walks in a line.

When the user walks for longer paths which include several line segments, there is a chance to further improve the accuracy and robustness.
In this case, we synthesize all the estimations by proposing the synchronizing scheme.
Specifically, the sine wave in the audio is modulated with periodical pulses.
The phone then detects and records the arrival time of these pulses.
In synthesizing, all estimations are used to compute the sent time of pulses.
Hence, when the computed sent time is accurate enough, the distance can be derived according to the receiving time and predicted sent time of the pulse, instead of the previous distance estimation.
Finally, the real-time position is computed.

We make performance evaluation on all the components with several types of cases and then the total performance of \ourprotocol.
%The extensive experiments show that the ranging and the direction estimation errors are under $0.66m$ and $5.06^o$ at the percentage of $90\%$ in most cases, when all the components of \ourprotocol are used.
The extensive experiments show that in position estimation, the ranging and angle errors is under $0.99m$ and $3.7^o$ at the percentage of $80\%$ correspondingly.
In synchronization, the successful detection rate is above $80\%$ for most cases and the corresponding standard deviation is around $10cm$.
For the total performance, the ranging errors are under $0.16m$, $0.32$, $0.54m$ at the percentage of $50\%$, $80\%$, $90\%$ correspondingly and the mean error is $0.71m$.
The angle errors are under $1.05^o$, $2.81^o$, $5.02^o$ at the percentage of $50\%$, $80\%$, $90\%$ correspondingly and the mean error is $2.20^o$.


The rest of the paper is organized as follows: we review the related work in Section \ref{sec:relatedwork} and present the overview of \ourprotocol in Section \ref{sec:overview}.
We propose the displacement tracking method in Section \ref{sec:pll} and then present the position estimation based on displacement tracking in Section \ref{sec:posest}.
We present the synchronization and synthesizing in Section \ref{sec:sync}.
We report our extensive experimental results in Section \ref{sec:exp}.
We conclude the paper in Section \ref{sec:conclusion}.


%In Figure \ref{fig:distance}, the user starts walking from $O_1$ and steps at $O_2$, $O_3, \dots, O_n$.
%$A$ is the position of the acoustic source.
%
%\begin{figure}[htpb]
%
%    \begin{center}
%        \includegraphics{fdistance1-crop.pdf}
%        %\caption{3D View}
%    \end{center}
%    \caption{3D View of the user walking straight forward.}
%    \label{fig:distance}
%%    \caption{(a) 3D View of the user walking straight forward. (b) Determining the side of the speaker.}
%%    \label{fig:bothest}
%\end{figure}
%Hence, 
%Recent advances in mobile computing enable smartphones for not only locating themselves, but also other people, \eg, Google's Latitude \cite{GoogleLatitude}, Facebook's Friendshake \cite{friendshake}. 
%However, such applications do not locate the people in proximity due to the limited accuracy or expensive infrastructure in indoor localization \cite{2012-MOBICOM-PushlimitWiFi}.
%It can be foreseen that wider applications are welcome if the problem is solved, for example, 
%positioning the person who broadcasts the common interest and making friends, 
%finding and picking up the guest at the airport, 
%following the guide in the touring party, 
%keeping an ``eye'' on children while shopping, 
%or locating the emergency exit or fire hydrant.

%Indoor localization is an important problem nowadays.
%However, recent solutions has limitations due to either the accuracy or the expense of deployment.
%For example, the WIFI localization only requires existing wireless routers that gathers the signal strength based on RSSI.
%However, the accuracy is limited and cannot be used for some cases, \eg, the supermarkets, libraries, museums and so on.
%Other techniques, such as TOA, TDOA, AOA, can reach considerable accuracy, but it requires specialized hardwares and additional infrastructures.
%To eliminate the above limitations, we propose a novel localization method by firstly answering the question:
%can we directly calculate the distance and direction from the smartphone to the commercial off-the-shelf (COTS) speaker, which has been installed in many public places? 
%
%However, both measurements are challenging to be obtained.
%Former ranging methods such as TOA or TDOA requires specialized hardwares or communications among entities to compute the accurate distance.
%The key problem is that the entities must be synchronized.
%For instance, when the receiver gets the signal from the sender, as the distance $l=v(t_r-t_s)$, where $t_s, t_r$ is the sending and receiving time correspondingly and $v$ is the travelling speed the signal.
%The reader directly get $t_r$ but needs technical ways to get $t_s$.
%%Hence, how to get $t_s$ from the speaker is the first challenging problem.
%There also have been methods in direction finding.
%But most of the implementations also require the special hardwares, such as antenna array or directional antenna. 
%
%In this paper, we propose and implement the indoor localization mechanism, \ourprotocol, which is based on the calculated position, \ie, the distance and direction, from the user to the speaker.
%The key insight is that when the user walks, the relative displacement from the phone to the speaker at each user's step is related to the position. 
%To track the real-time displacement, we mix a non-audible continuas sine signal into the acoustic wave of the speaker, and adopt the second-order phase locked loop (PLL) to track the phase shift of the signal, which correpsonds to the relative displacement.
%Then the position is estimated according to relative displacement and walking length of the user's steps.
%Note that accuracy of the estimation also varies according to different positions and can be improved by synthesizing all the estimations.
%Hence, we further propose the synchronizing and the corresponding ranging method.
%Specifically, we modulate periodical pulses into the sine signal for synchronization and synthesizing.
%Once the historical distance is calculated, the sending time of the pulse can be predicted also by synchronization, and the latter distance is directly obtained without estimation. 
%After the real-time direction is also obtained, the location of the user is inferred from the position of the speaker, and the accuracy is enhanced if more speakers are detected.
%
%The contributions of the paper are as follows:
%\begin{itemize}
%    \item We propose a novel speaker positioning method by leveraging the accurate relative displacement when the phone user walks.
%        To the best of our knowledge, it is the first try to measure the position of the raw speakers.
%    \item We adopt the second-order PLL to track the accurate real-time relative displacement when the acoustic signal is weak.
%    \item We propose pulse modulating and the corresponding synchoronization mechanism, where the pulse takes very narrow bandwidth and can be accurately detected when the signal is weak.
%    \item We implement \ourprotocol based on the speaker positioning, which achieves high accuracy and does not require any special infrastructures in many public places.
%\end{itemize}
%
%





==> toverview-old.tex <==
\section{Architecture Overview DELETED}
\label{sec:overview-old}


The key insight of our paper is that when a user walks along a line, the pattern of displacements
 from the user to an acoustic speaker is related to relative position directly.
%Let us take the case shown in Figure \ref{fig:example} as an example.
For example in Figure \ref{fig:example}, a user walks and steps at $O_1$, $O_2$, and $O_3$.
The displacements $d_1$(=$l_1-l_2$) and $d_2$(=$l_2-l_3$) are measured respectively
 and the user's stride length ($|\overline{O_1O_2}|$) is given.
Intuitively, $d_1\approx0$ infers that $O_1$ and $O_2$ are close to $H$ where $\overline{AH} \bot \overline{O_1O_2}$ and $d_2<0$,
 which tells us that the speaker is at the back of the walking user,
 hence infers the coarse-grained direction.
Another observation is that when the distance $|\overline{AH}|$ increases, the value of 
 $|d_2-d_1|$ decreases, which infers the coarse-grained distance as well.
So, the relative position between the speaker $A$ and the piecewise linear segment $\overline{O_1O_3}$ can be computed.
Clearly, in this case, if the speaker serves as an anchor and its coordinate in the room is given, the real-time position of the user (\eg, $O_1$, $O_2$, $O_3$,\dots) can be inferred directly, and vice versa.
However, when $|\overline{AH}|$ becomes much larger, $|d_2-d_1|$ is much smaller which results in less accurate measurement by leveraging this property. Hence, we use synchronization to enhance the accuracy and robustness.

Note that to the best of our knowledge, current approaches cannot directly obtain distances $l_1$ without synchronization between the receiver and the dummy speaker.
They require additional capabilities of the speaker, such as communication capability that exchanges synchronization information \cite{2007-SenSys-BeepBeephighaccuracy}.
Instead, we calculate the displacement $d=l_1-l_2$ by PLL.


%\ourprotocol is a precise ranging and direction estimation scheme that calculates the real-time position of the acoustic speaker when the user walks.
%Based on the above insight, we show the architecture of \ourprotocol in Figure \ref{fig:overview}. 
%{\color{red}TODO: add explanation of synchronization}

In synchronization, our main purpose is to take advantage of historical samples to improve robustness and accuracy. 
Once a good estimation of distance is obtained from historical result, the latter distances can be precisely obtained in case of even longer distances. 
Specifically, we add periodical pulses to the sending signal, where the sending time of the pulse is unknown and solved by synthesizing the historical samples.
Then, the sending time is used to directly calculate the latter distances according the difference from the receiving time to the sending time.


We show the architecture of \ourprotocol in Figure \ref{fig:overview}. 
\ourprotocol consists of the following steps:
\begin{enumerate}
    \item The dummy speaker broadcasts audio mixed with modulated non-audible wave. 
        The main component is the high-frequency sine wave which is used to track the displacement in step 2.
        We also modulate the sine wave with periodical pulses for every 0.25 seconds.
        It is used for synchronization in step 4.
    \item The smart device uses the second-order Phase Locked Loop (PLL) to track the phase derived from the wave, which corresponds to the displacement from the phone to the user when the user walks.
        Note that the received signal goes through Band-Pass Filter (BPF) and Automatic Gain Control (AGC) before it is tracked by PLL \cite{DBLP:journals/corr/HuangXLLMYL13}.
        %Readers interested in design of BPF and AGC can refer to \cite{DBLP:journals/corr/HuangXLLMYL13}.
    \item In case that the user walks and the distance within $8m$, \ourprotocol estimates the distance from the speaker to the piecewise linear segment.
        Then relative position from the user to the dummy speaker at each step of the linear segment is also estimated.
        For estimating the location of the user, we not only use the displacement stemmed from step 2, but also the user's walking time, which is detected by Inertial Measurement Unit (IMU) of smart phones. 
        Note that the accuracy of this estimation is unstable due to different relative positions and lengths of the linear segment. 
        To remedy the deficiencies, \ourprotocol further improves the accuracy and robustness in step 4.
    \item \ourprotocol detects the periodical pulses and calculates the precise receiving time.
        \ourprotocol then computes the sending time of the pulses by synthesizing all the results in step 3.
        More specifically, as the localization accuracy in step 3 for each walking segment is different, we choose the location result of the more accurate one.
        Then, we infer the sending time of each periodical pulses by using the arrival time of the pulses and the distance which is inferred from the location result.
        When the sending time of the pulses is accurately calculated, the real-time distance is no longer calculated in step 3, but by using the accurate predicted sending time and newly detected received time of the pulse.
        Finally, the real-time distance and the direction are computed.
        %We call this step the synchronization as it solve the ranging problem which is based on synchronization in most literatures.
\end{enumerate}

%Note that the compass of the smartphone is sensitive to the surrounding environment, the calculated direction has errors which affects the accuracy of indoor localization, especially when there is only one detectable speaker around.
%As a result, we design particle filter and leverage the indoor map to calibrate the natural error of the compass. 
%


